Limit Laws for Empirical Optimal Solutions in Stochastic Linear Programs

We consider a general linear program in standard form whose right-hand side constraint vector is subject to random perturbations. This defines a stochastic linear program for which, under general conditions, we characterize the fluctuations of the corresponding empirical optimal solution by a central limit-type theorem. Our approach relies on the combinatorial nature and the concept of degeneracy inherent in linear programming, in strong contrast to well-known results for smooth stochastic optimization programs. In particular, if the corresponding dual linear program is degenerate the asymptotic limit law might not be unique and is determined from the way the empirical optimal solution is chosen. Furthermore, we establish consistency and convergence rates of the Hausdorff distance between the empirical and the true optimality sets. As a consequence, we deduce a limit law for the empirical optimal value characterized by the set of all dual optimal solutions which turns out to be a simple consequence of our general proof techniques. Our analysis is motivated from recent findings in statistical optimal transport that will be of special focus here. In addition to the asymptotic limit laws for optimal transport solutions, we obtain results linking degeneracy of the dual transport problem to geometric properties of the underlying ground space, and prove almost sure uniqueness statements that may be of independent interest.

==> Sections/Illustration.tex <==
\section{Optimal Transport -- Illustration}\label{sec:illustration}

In this section, we illustrate the central limit theorem in Theorem \ref{thm:limitGeneral} and the Hausdorff distance approximation in Theorem \ref{thm:Hausdorff} for an instance of the optimal transport problem. More specifically, we choose the ground space $\mathcal{X}=\{x_1<x_2<x_3\}$ to be three points on the real line with cost $c(x_i,x_j)=\vert x_i-x_j\vert^p$ for $p>0$. For two probability vectors $r,s\in\Delta_3$ on $\mathcal{X}$, the optimal transport problem \eqref{eq:OTprimal} reads
\begin{small}
\begin{equation*}
\begin{aligned}
\min_{\pi\in\mathbb{R}^9} \quad
c^T\pi& \\
\text{s.t.} \quad
\pi\in \Pi_{\dagger}(r,s)\coloneqq &\left\lbrace \pi\in \mathbb{R}^{9}\,\vert\, A_{\dagger}\pi=\begin{bmatrix}
r_{\dagger}\\s
\end{bmatrix},\,\pi\geq 0  \right\rbrace
\end{aligned}
\end{equation*}
\end{small}
with cost vector 
\begin{small}
\begin{equation*}
\begin{split}
c
%&=\mathrm{Vec}
%\begin{pmatrix}
%0&\vert x_2-x_1\vert^p&\vert x_3-x_1\vert^p\\
%(x_2-x_1)^p&0&(x_3-x_2)^p\\
%(x_3-x_1)^p&(x_3-x_2)^p&0
%\end{pmatrix}\\
&=\left(0,\vert x_1-x_2\vert^p,\vert x_1-x_3\vert^p,
\vert x_2-x_1\vert^p,0,\vert x_2-x_3\vert^p,
\vert x_3-x_1\vert^p,\vert x_3-x_2\vert^p,0\right)\in \mathbb{R}^9
\end{split}
\end{equation*}
\end{small}
and constraint or node-arc incidence matrix
\begin{small}
\begin{equation*}
A_\dagger =
\begin{pmatrix}
1&1&1\\
&&&1&1&1\\
1 &&& 1 &&& 1 \\
&1&&& 1 &&& 1\\
&& 1&&& 1 &&& 1\\
\end{pmatrix}\in \mathbb R^{5\times 9}.
\end{equation*}
\end{small} 
A basis $I$ is a subset of cardinality five out of the column index set $\{1,\ldots,9\}$ from $A_\dagger$ such that the sub-matrix ${A_\dagger}_I$ contains five independent columns. For example, the subset $I=\{1,2,3,5,9\}$ constitutes a basis. For optimal transport it is convenient to think of a primal feasible solution in terms of a transport matrix $\pi \in \mathbb{R}^{3\times 3}$ with $\pi_{ij}$ encoding mass transportation from source $i$ to destination $j$. In this way, a basis $I$ can be identified with its \textit{transport scheme} of primal basic feasible transport matrices. More precisely, the above basis $I$ corresponds to the transport scheme
\begin{small}
\begin{equation*}
TS(I)\coloneqq\begin{pmatrix}
\ast & \ast & \ast\\
 & \ast\\
&&\ast\\
\end{pmatrix}.
\end{equation*}
\end{small}
Each nonzero entry is marked by a star and the specific values are defined by $\pi(I,(r_\dagger,s))=({A_\dagger}_I)^{-1}(r_\dagger,s)\in\mathbb{R}^9$. In particular, the above transport scheme yields a primal basic feasible solution if and only if each nonzero coordinate is nonnegative. For instance and by a slight abuse of notation, basis $I$ induces the primal basic feasible solution
\begin{small}
\begin{equation*}
\pi\left(I,(r_\dagger,s)\right)=\begin{pmatrix}
s_1 & s_2-r_2 & r_1+r_2-s_1-s_2\\
& r_2\\
&&s_1+s_2+s_3-r_1-r_2
\end{pmatrix}=\begin{pmatrix}
s_1 & s_2-r_2 & s_3-r_3\\
& r_2\\
&&r_3
\end{pmatrix},
\end{equation*}
\end{small}
where for the second equality we specifically use that the probability vectors $r,s$ sum up to one, respectively. By nonnegativity, $\pi\left(I,(r_\dagger,s)\right)$ is feasible if and only if $s_2\geq r_2$ and $s_3\geq r_3$.

\textbf{The Limit Law.} Assume that the two probability vectors are equal and strictly positive: $r=s>0$. Then the transport problem attains a unique solution supported on the diagonal, i.e., all the mass remains at its current location. In particular, the optimal solution is degenerate. For our case of 9 variables and 5 constraints, there are at most $\binom 95=126$ candidates for bases $I$. In this one-dimensional optimal transport problem, however, only 81 are such that the corresponding matrix $A_{\dagger I}$ is invertible. Moreover and since the optimal solution is supported on the diagonal, each primal optimal basis necessarily includes the diagonal. In terms of the bases set that means that for each primal and dual optimal basis $\{1,5,9\}\subset I$, and only such bases could appear in the limit law. There are at most twelve such bases, corresponding to the transport schemes

\begin{small}
\begin{tabular}{cccc}
$TS(I_1)=\begin{pmatrix}
\ast & \ast \\
&\ast&\\
&\ast&\ast
\end{pmatrix}$ & $TS(I_2)=\begin{pmatrix}
\ast &  \\
\ast&\ast&\ast\\
&&\ast
\end{pmatrix}$ & $TS(I_3)=\begin{pmatrix}
\ast & & \\
\ast & \ast& \\
\ast & &\ast
\end{pmatrix}$ & $TS(I_4)=\begin{pmatrix}
\ast & &\ast \\
 & \ast&\ast \\
 & &\ast
\end{pmatrix}$ \\ 
$TS(I_5)=\begin{pmatrix}
\ast & \ast & \ast \\
&\ast&\\
&&\ast
\end{pmatrix}$ & $TS(I_6)=\begin{pmatrix}
\ast &&  \\
&\ast&\\
\ast&\ast&\ast
\end{pmatrix}$ & $TS(I_7)=\begin{pmatrix}
\ast &  \\
\ast&\ast&\\
&\ast&\ast
\end{pmatrix}$ & $TS(I_8)=\begin{pmatrix}
\ast & \ast \\
&\ast&\ast\\
&&\ast
\end{pmatrix}$ \\
$TS(I_{9})=\begin{pmatrix}
\ast & &\ast \\
& \ast &\\
&\ast&\ast
\end{pmatrix}$ & $TS(I_{10})=\begin{pmatrix}
\ast && \ast \\
\ast&\ast\\
&&\ast
\end{pmatrix}$ & $TS(I_{11})
=\begin{pmatrix}
\ast & & \\
 &\ast &\ast \\
\ast & &\ast
\end{pmatrix}$ & $TS(I_{12})
=\begin{pmatrix}
\ast &\ast & \\
 &\ast & \\
\ast & &\ast
\end{pmatrix}$, \\ 
\end{tabular} 
\end{small}

all of which are optimal for $r=s$. Which of these bases also induce dual optimal basic solutions depends on the cost vector $c$ through the parameter $p>0$. Recalling that $K$ is the number of bases that are primal and dual feasible, we obtain for this example:

\begin{table}[h!]
\begin{center}
\begin{tabular}{c|c|c}
\renewcommand{\arraystretch}{1.5}
$p$ & primal \& dual optimal bases & $K$\\
\hline
$(0,1)$ & $I_1$, $I_2$, $I_3$, $I_4$, $I_5$, $I_6$ & 6\\
1 & $I_1$, $I_2$, $I_3$, $I_4$, $I_5$, $I_6$, $I_7$, $I_8$ & 8\\
$(1,\infty)$ & $I_1$, $I_2$, $I_7$, $I_8$ & 4\\
\end{tabular}
\caption{Primal and dual optimal bases for optimal transport between three ordered points on the real line. Cost given by $\vert x-y\vert^p$ depending on $p$.}
\end{center}
\end{table}
Bases $I_9$, $I_{10}$, $I_{11}$ and $I_{12}$ do not appear, as these are dual infeasible for all $p>0$. Hence, we only need to consider bases $I_1,\ldots,I_8$. Computing all corresponding closed convex cones $H_k$ for $1\leq k\leq 8$ as defined in \eqref{eq:Hk} yields

\begin{small}
\begin{align*}
H_{1}&=\left\lbrace v\in \mathbb{R}^5\, \mid \, v_1\geq v_3,\, v_1+v_2\leq v_3+v_4\right\rbrace,\quad H_{2}=\left\lbrace v\in \mathbb{R}^5\, \mid \, v_1\leq v_3,\, v_1+v_2\geq v_3+v_4\right\rbrace,\\
H_{3}&=\left\lbrace v\in \mathbb{R}^5\, \mid \, v_2\geq v_4,\, v_1+v_2\leq v_3+v_4\right\rbrace,\quad H_{4}=\left\lbrace v\in \mathbb{R}^5\, \mid \, v_1\geq v_3,\, v_2\geq v_4\right\rbrace,\\
H_{5}&=\left\lbrace v\in \mathbb{R}^5\, \mid \, v_2\leq v_4,\, v_1+v_2\geq v_3+v_4\right\rbrace,\quad H_{6}=\left\lbrace v\in \mathbb{R}^5\, \mid \, v_1\leq v_3,\, v_2\leq v_4\right\rbrace,\\
H_{7}&=\left\lbrace v\in \mathbb{R}^5\, \mid \, v_1\leq v_3,\, v_1+v_2\leq v_3+v_4\right\rbrace, \quad H_{8}=\left\lbrace v\in \mathbb{R}^5\, \mid \, v_1\geq v_3,\, v_1+v_2\geq v_3+v_4\right\rbrace.
\end{align*}
\end{small}
Recall the limit law in \eqref{eq:empprocess2} for the probability vectors $\left(r_\dagger,s\right)$, given by
\begin{small}
\begin{equation*}
\sqrt{\frac{nm}{n+m}}\left( \begin{bmatrix}
\hat{r_\dagger}_n\\ \hat{s}_m
\end{bmatrix}-\begin{bmatrix}
r_\dagger\\ s
\end{bmatrix} \right) \xrightarrow[]{D} \left( \sqrt{\lambda}G^1(r_\dagger),\sqrt{1-\lambda}G^2(s)\right) = \mathbf{G}\in \mathbb{R}^5.
\end{equation*}
\end{small}
Straightforward computations show that the nondegeneracy assumption \eqref{ass:dualnondegen} holds for all $p\neq 1$.
We deduce that according to Theorem \ref{thm:limitforOT} the limit law for optimal transport couplings in the case $r=s$ for $p\in (1,\infty)$ is given by $K=4$ summands 
\begin{small}
\begin{equation*}
\begin{split}
M(\mathbf{G})=\sum_{k\in\{1,2,7,8\}}&\mathbbm{1}_{\mathbf{G}\in H_{k}}\pi(I_k,\mathbf{G})=\\
&\mathbbm{1}_{\left\lbrace\substack{\mathbf{G_1}\geq \mathbf{G_3}\\ \mathbf{G_1}+\mathbf{G_2}\leq\mathbf{G_3}+\mathbf{G_4} }\right\rbrace}\pi(I_1,\mathbf{G})+
\mathbbm{1}_{\left\lbrace\substack{\mathbf{G_1}\leq \mathbf{G_3}\\ \mathbf{G_1}+\mathbf{G_2}\geq \mathbf{G_3}+\mathbf{G_4}}\right\rbrace}\pi(I_2,\mathbf{G})+\\
&\mathbbm{1}_{\left\lbrace\substack{\mathbf{G_1}\leq \mathbf{G_3}\\  \mathbf{G_1}+\mathbf{G_2}\leq \mathbf{G_3}+\mathbf{G_4}}\right\rbrace}\pi(I_7,\mathbf{G})+
\mathbbm{1}_{\left\lbrace\substack{\mathbf{G}_1\geq \mathbf{G_3}\\  \mathbf{G_1}+\mathbf{G_2}\geq \mathbf{G_3}+\mathbf{G_4}}\right\rbrace}\pi(I_8,\mathbf{G}).
\end{split}
\end{equation*}
\end{small}

Similarly, the limit law for $p\in (0,1)$ contains $K=6$ summands and is given by

\begin{small}
\begin{equation*}
M(\mathbf{G})=\sum_{1\leq k\leq 6}\mathbbm{1}_{\mathbf{G}\in H_{k}}\pi(I_k,\mathbf{G}).
\end{equation*}
\end{small}

A more interesting and complex situation arises for $p=1$. In this case assumption \eqref{ass:dualnondegen} fails and the indicator functions in the limit law now require intersections of closed convex cones corresponding to bases that induce the same primal optimal basic solution. This is the case for the pairs of bases $\{I_3,I_7\}$, $\{I_6,I_7\}$, $\{I_4,I_8\}$ and $\{I_5,I_8\}$. The intersections of the corresponding cones are given by 
\begin{small}
\begin{align*}
H_3\cap H_7&=\left\lbrace v\in \mathbb{R}^5\, \mid \, v_2\geq v_4,\, v_1+v_2\leq v_3+v_4\right\rbrace,\\
H_6\cap H_7&=\left\lbrace v\in \mathbb{R}^5\, \mid \, v_1\leq v_3,\, v_2\leq v_4\right\rbrace,\\
H_4\cap H_8&=\left\lbrace v\in \mathbb{R}^5\,\mid\, v_1\geq v_3,\, v_2\geq v_4 \right\rbrace,\\ 
H_5\cap H_8&=\left\lbrace v\in\mathbb{R}^5\, \mid \, v_2\leq v_4, \, v_1+v_2\geq v_3+v_4 \right\rbrace.
\end{align*}
\end{small}

Hence, the limit law for $p=1$ and $r=s$ reads 
\begin{equation*}
M(\mathbf{G})=\sum_{\K\in\{\{1\},\{2\}\{3,7\},\{6,7\},\{4,8\},\{5,8\}\}} \mathbbm{1}_{\mathbf{G}\in H_\K\setminus\cup_{k\notin\K}H_k}\,\alpha^\K \otimes x(I_\K,G).
\end{equation*}

This combinatorial structure of the limit law depends on the convexity $(p>1)$ or concavity $(0<p<1)$ of the cost function but neither on the exact value of $p$ nor on the position of the points $x_1<x_2<x_3$.

\textbf{The Hausdorff Distance.} Suppose now that $p=1$ but the probability vectors are $r=\left(\nicefrac{1}{4},\nicefrac{1}{4},\nicefrac{1}{2}\right)$ and $s=\left(\nicefrac{1}{2},\nicefrac{1}{4},\nicefrac{1}{4}\right)$. In this case, there are four primal and dual optimal transport schemes $I_1,I_2,I_3,I_4$, namely

\begin{small}
\begin{center}
\begin{tabular}{cc}
$TS(I_1)=\begin{pmatrix}
\ast & & \\
\ast& &\\
\ast&\ast&\ast
\end{pmatrix}$, & $TS(I_2)=\begin{pmatrix}
\ast & & \\
\ast&\ast&\\
&\ast&\ast
\end{pmatrix}$, \\ 
$TS(I_3)=\begin{pmatrix}
\ast & & \\
&\ast&\\
\ast&\ast&\ast
\end{pmatrix}$, & $TS(I_4)=\begin{pmatrix}
\ast &  \\
\ast&\ast&\\
\ast& &\ast
\end{pmatrix},$ \\ 
\end{tabular} 
\end{center}
\end{small}
that induce the following two primal optimal basic solutions
\begin{small}
\begin{equation*}
\begin{split}
\pi(I_1,(r_\dagger,s))=\pi(I_2,(r_\dagger,s))&=\begin{pmatrix}
\nicefrac{1}{4} & & \\
\nicefrac{1}{4}&0 &\\
0&\nicefrac{1}{4}&\nicefrac{1}{4}
\end{pmatrix}\, ,\\
\pi(I_3,(r_\dagger,s))=\pi(I_4,(r_\dagger,s))&=\begin{pmatrix}
\nicefrac{1}{4} &  \\
0&\nicefrac{1}{4}&\\
\nicefrac{1}{4}&0 &\nicefrac{1}{4}
\end{pmatrix},
\end{split}
\end{equation*}
\end{small}
respectively. Notice that each convex combination of both primal optimal basic solutions is also primal optimal. According to our equivalence classes as defined in the proof of Theorem \ref{thm:Hausdorff} in Proof \ref{proof:Hausdorff}, we find that $\mathcal{B}_1=\{1,2\}$ and $\mathcal{B}_2=\{3,4\}$. Suppose for $\varepsilon>0$ sufficiently small we perturb the probability vector $r$ to obtain $\tilde{r}=\left(\nicefrac{1}{4}+\varepsilon,\nicefrac{1}{4}-\varepsilon,\nicefrac{1}{2}\right)$. By the nonnegativity constraint the transport scheme $I_4$ becomes infeasible:
\begin{small}
\begin{equation*}
\pi(I_4,(\tilde{r}_\dagger,s))=\begin{pmatrix}
\nicefrac{1}{4}+\varepsilon &  \\
-\varepsilon & \nicefrac{1}{4} &\\
\nicefrac{1}{4}&0 &\nicefrac{1}{4}
\end{pmatrix}.
\end{equation*}
\end{small}
However, for $\varepsilon\in (0,\nicefrac{1}{4})$ the transport schemes $I_1,I_2,I_3$ remain feasible:
\begin{small}
\begin{equation*}
\begin{split}
\pi(I_1,(\tilde{r}_\dagger,s))=\pi(I_2,(\tilde{r}_\dagger,s))&=\begin{pmatrix}
\nicefrac{1}{4}+\varepsilon & & \\
\nicefrac{1}{4}-\varepsilon &0 &\\
0&\nicefrac{1}{4}&\nicefrac{1}{4}
\end{pmatrix}\, ,\\
\pi(I_3,(\tilde{r}_\dagger,s))&=\begin{pmatrix}
\nicefrac{1}{4}+\varepsilon &  \\
0&\nicefrac{1}{4}-\varepsilon&\\
\nicefrac{1}{4}-\varepsilon& \varepsilon &\nicefrac{1}{4}
\end{pmatrix},
\end{split}
\end{equation*}
\end{small}
and hence optimal. As expected from Lemma \ref{lem:basisequivalenceclasses}, for small perturbations at least one transport scheme from each equivalence class $\mathcal{B}_1$, $\mathcal{B}_2$ remains optimal for the perturbed problem. In addition to optimality of $I_1$, $I_2$ and $I_3$, it is clear that
\begin{equation*}
\Vert \pi(I_j,(r_\dagger,s))-\pi(I_j,(\tilde{r}_\dagger,s))\Vert=O(\varepsilon)
\end{equation*}
for $j=1,2,3$. Although for the perturbed problem $I_4$ is no longer feasible, we still have $\Vert \pi(I_4,(r_\dagger,s))-\pi(I_3,(\tilde{r}_\dagger,s))\Vert=O(\varepsilon)$. In particular, we conclude for the Hausdorff distance 
\begin{equation*}
d_H\left(Opt\left(r_\dagger,s\right),Opt\left(\tilde{r}_\dagger,s\right)\right)=O(\varepsilon).
\end{equation*}
For small perturbations with $\epsilon<0$, then $I_1$, $I_2$ and $I_4$ are optimal and $I_3$ becomes infeasible.  In a similar fashion to aforementioned case, it holds that $\Vert \pi(I_3,(r_\dagger,s))-\pi(I_4,(\tilde{r}_\dagger,s))\Vert=O(\varepsilon)$ and the Hausdorff distance between the optimality sets is $O(\varepsilon)$. Thus the Hausdorff distance is of the same magnitude as the perturbations, which is $O_\mathbb P(r_n^{-1})$ in view of \eqref{ass:cltforb}.

